Savaal: Scalable Concept-Driven Question Generation to Enhance Human Learning

Assessing and enhancing human learning through question-answering is vital, yet automating this process remains challenging. While large language models (LLMs) excel at summarization and query responses, their ability to generate meaningful questions for learners is underexplored. We propose Savaal, a scalable question-generation system with three objectives: (i) scalability, enabling question generation from hundreds of pages of text (ii) depth of understanding, producing questions beyond factual recall to test conceptual reasoning, and (iii) domain-independence, automatically generating questions across diverse knowledge areas. Instead of providing an LLM with large documents as context, Savaal improves results with a three-stage processing pipeline. Our evaluation with 76 human experts on 71 papers and PhD dissertations shows that Savaal generates questions that better test depth of understanding by 6.5X for dissertations and 1.5X for papers compared to a direct-prompting LLM baseline. Notably, as document length increases, Savaal's advantages in higher question quality and lower cost become more pronounced.

==> 110scalability.tex <==
\subsection{Cost Analysis}
\label{appendix:scalability}

We define the \emph{cost} of the system as the total number of input and output tokens used to generate $N$ questions by $\text{Cost}(N)$, and we inspect how $\text{Cost}(N)$ grows as $N$ increases. \\


\NewPara{Cost when using the Entire Document}: Assume that in each question generation round, we use a \emph{question batch size} of $b$ -- i.e., LLM is prompted to generate $b$ questions. If the average number of input tokens is $D$ and the average number of output tokens per question is $q$, using the entire document to generate $N$ questions would result in {\small $\text{Cost}_{\text{Entire Document}}(N) = \frac{N}{b} D + N q$}. 
Note that this system has a running cost of processing the document proportional to $N$ (i.e., $\frac{N}{b} D$). \\


\NewPara{Cost when using a pre-processed text}: When using a preprocessed text This system has a fixed one-time cost for generating the summary denoted by $f(D)$. If the avg number tokens in the summary is denoted by $D_{s}$ and the batch size of $b_s$ is used, we have {\small $Cost_{\textit{Summary}}(N) = f(D) + \frac{N}{b_s} D_{s} + N q$}. Note that as $N$ grows, we have: 

\begin{small}
\begin{align}
    \lim_{N \rightarrow \infty} & \big( \text{Cost}_{\textit{Entire Document}}(N) 
    - \text{Cost}_{\textit{Summary}}(N) \big) \nonumber \\
    &= N \left(\frac{D}{b} - \frac{D_{s}}{b_s}\right)- f(D) \nonumber \\
    &= N \left(\frac{D}{b} - \frac{D_{s}}{b_s}\right) \nonumber \\
\label{eqn:scalability}
\end{align}
\end{small}

In words, if $\frac{D_{s}}{b_s} < \frac{D}{b}$, as the number of questions increases, the cost of the system using the entire document is much larger than the system using the summary -- the cost difference in \autoref{eqn:scalability} grows to infinity.
 

